Mosaic: An Application-Transparent Hardware-Software Cooperative Memory Manager for GPUs

Modern GPUs face a trade-off on how the page size used for memory management affects address translation and demand paging. Support for multiple page sizes can help relax the page size trade-off so that address translation and demand paging optimizations work together synergistically. However, existing page coalescing and splintering policies require costly base page migrations that undermine the benefits multiple page sizes provide. In this paper, we observe that GPGPU applications present an opportunity to support multiple page sizes without costly data migration, as the applications perform most of their memory allocation en masse (i.e., they allocate a large number of base pages at once). We show that this en masse allocation allows us to create intelligent memory allocation policies which ensure that base pages that are contiguous in virtual memory are allocated to contiguous physical memory pages. As a result, coalescing and splintering operations no longer need to migrate base pages. We introduce Mosaic, a GPU memory manager that provides application-transparent support for multiple page sizes. Mosaic uses base pages to transfer data over the system I/O bus, and allocates physical memory in a way that (1) preserves base page contiguity and (2) ensures that a large page frame contains pages from only a single memory protection domain. This mechanism allows the TLB to use large pages, reducing address translation overhead. During data transfer, this mechanism enables the GPU to transfer only the base pages that are needed by the application over the system I/O bus, keeping demand paging overhead low.

==> confnames.tex <==
\newboolean{longconferencenames}
\setboolean{longconferencenames}{true}

\ifthenelse{\boolean{longconferencenames}}
{
\newcommand{\uss}{USENIX Security Symposium}
\newcommand{\hotsec}{USENIX Workshop on Hot Topics in Security (HotSec)}
\newcommand{\ccs}{ACM Conference on Computer and Communications Security (CCS)}
\newcommand{\cacm}{Communications of the {ACM}(CACM)}
\newcommand{\sandp}{IEEE Symposium on Security and Privacy}
\newcommand{\sosp}{ACM Symposium on Operating System Principles (SOSP)}
\newcommand{\osdi}{USENIX Symposium on Operating Systems Design and Implementation (OSDI)}
\newcommand{\eurosys}{ACM European Conference in Computer Systems (EuroSys)}
\newcommand{\hotos}{USENIX Workshop on Hot Topics in Operating Systems (HotOS)}
\newcommand{\popl}{Symposium on Principles of Programming Languages (POPL)}
\newcommand{\ndss}{Network and Distributed System Security Symposium (NDSS)}
\newcommand{\blackhat}{Black Hat Technical Security Conference}
\newcommand{\dsn}{IEEE/IFIP International Conference on Dependable Systems and Networks (DSN)}
\newcommand{\dimva}{Detection of Intrusions and Malware and Vulnerability Assessment (DIMVA)}
\newcommand{\raid}{International Symposium on Recent Advances in Intrusion Detection (RAID)}
\newcommand{\isca}{International Symposium on Computer Architecture (ISCA)}
\newcommand{\asplos}{International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}
\newcommand{\vb}{Virus Bulletin Conference}
\newcommand{\webapps}{USENIX Conference on Web Application Development (WebApps)}
\newcommand{\acsac}{Annual Computer Security Applications Conference (ACSAC)}
\newcommand{\wisa}{International Workshop on Information Security Applications (WISA)}
\newcommand{\most}{Mobile Security Technologies (MoST)}
\newcommand{\wisec}{ACM Conference on Security and Privacy in Wireless and Mobile Networks (WiSec)}
\newcommand{\www}{International World Wide Web Conference (WWW)}
\newcommand{\mobisys}{The International Conference on Mobile Systems, Applications, and Services (MobiSys)}
\newcommand{\tissec}{ACM Transactions on Information and System Security (TISSEC)}
\newcommand{\hotmobile}{International Workshop on Mobile Computing Systems and Applications (HotMobile)}
\newcommand{\isc}{Information Security Conference (ISC)}
\newcommand{\asiaccs}{ACM Symposium on Information, Computer and Communications Security (AsiaCCS)}
\newcommand{\icdcs}{IEEE International Conference on Distributed Computing Systems (ICDCS)}
\newcommand{\sigmetrics}{ACM International Conference on Measurement and Modeling of Computer Systems (SIGMETRICS)}
\newcommand{\sigmod}{ACM SIGMOD International Conference on Management of Data (SIGMOD)}
\newcommand{\vldb}{International Conference on Very Large Data Bases (VLDB)}
\newcommand{\oakland}{{Proceedings of the IEEE Symposium on Security and Privacy (Oakland)}}
\newcommand{\micro}{International Symposium on Microarchitecture}
\newcommand{\nsdi}{USENIX Symposium on Networked System Design and Implementation}
\newcommand{\hpca}{IEEE International Symposium on High Performance Computer Architecture (HPCA)}
}{
\newcommand{\uss}{USENIX Security}
\newcommand{\hotsec}{HotSec}
\newcommand{\ccs}{CCS}
\newcommand{\cacm}{CACM}
\newcommand{\sandp}{S\&P}
\newcommand{\sosp}{SOSP}
\newcommand{\osdi}{OSDI}
\newcommand{\hotos}{HotOS}
\newcommand{\eurosys}{EuroSys}
\newcommand{\popl}{POPL}
\newcommand{\ndss}{NDSS}
\newcommand{\blackhat}{Black Hat}
\newcommand{\dsn}{DSN}
\newcommand{\dimva}{DIMVA}
\newcommand{\raid}{RAID}
\newcommand{\isca}{ISCA}
\newcommand{\asplos}{ASPLOS}
% Not abbreviating, people may not know these
\newcommand{\vb}{Virus Bulletin Conference}
\newcommand{\webapps}{USENIX WebApps}
\newcommand{\acsac}{ACSAC}
\newcommand{\wisa}{WISA}
\newcommand{\most}{MoST}
\newcommand{\wisec}{WiSec}
\newcommand{\www}{WWW}
\newcommand{\mobisys}{MobiSys}
\newcommand{\tissec}{TISSEC}
\newcommand{\hotmobile}{HotMobile}
\newcommand{\isc}{ISC}
\newcommand{\asiaccs}{ASIACCS}
\newcommand{\icdcs}{ICDCS}
\newcommand{\sigmetrics}{SIGMETRICS}
\newcommand{\sigmod}{SIGMOD}
\newcommand{\vldb}{VLDB}
\newcommand{\oakland}{IEEE S\&P}
\newcommand{\micro}{MICRO}
\newcommand{\nsdi}{NSDI}
\newcommand{\hpca}{HPCA}
}

